The Bottleneck Simulator: A Model-based Deep Reinforcement Learning Approach

Deep reinforcement learning has recently shown many impressive successes. However, one major obstacle towards applying such methods to real-world problems is their lack of data-efficiency. To this end, we propose the Bottleneck Simulator: a model-based reinforcement learning method which combines a learned, factorized transition model of the environment with rollout simulations to learn an effective policy from few examples. The learned transition model employs an abstract, discrete (bottleneck) state, which increases sample efficiency by reducing the number of model parameters and by exploiting structural properties of the environment. We provide a mathematical analysis of the Bottleneck Simulator in terms of fixed points of the learned policy, which reveals how performance is affected by four distinct sources of error: an error related to the abstract space structure, an error related to the transition model estimation variance, an error related to the transition model estimation bias, and an error related to the transition model class bias. Finally, we evaluate the Bottleneck Simulator on two natural language processing tasks: a text adventure game and a real-world, complex dialogue response selection task. On both tasks, the Bottleneck Simulator yields excellent performance beating competing approaches.

==> old_long_related_work.tex <==
\section{Related Work}

\textbf{Model-based Reinforcement Learning}:

Early model-based reinforcement learning research dates back to the 90s, and include well-known algorithms such as Dyna, R-max and $\text{E}^3$~\citep{sutton1990integrated,moore1993prioritized,peng1993efficient,kuvayev1997approximation,brafman2002r,kearns2002near,wiering1998efficient,wiering1999reinforcement}.
Model-based reinforcement learning with deep learning has also been investigated, in particular for robotic control tasks~\citep{watter2015embed,lenz2015deepmpc,gu2016continuous,finn2017deep}.
Data efficient approaches have also been proposed by taking a Bayesian approach to learning the dynamics model. For example, PILCO incorporates uncertainty by learning a distribution over dynamics models in conjunction with the agent's policy~\citep{deisenroth2011pilco}.
Another approach based on Bayesian optimization was proposed by~\citet{bansal2017goal}.
An approach combining dynamics models of various levels of fidelity or accuracy (e.g.\@ combining a learned dynamics model with real-world samples) was proposed by~\citet{cutler2015real}.
Other related work includes~\citet{venkatraman2016improved}, ~\citet{kansky2017schema} and ~\citet{racaniere2017imagination}.
%Other related work includes\citet{bansal2017goal,cutler2015real}.

The idea of grouping similar states together also has a long history in the reinforcement learning community.
Numerous algorithms exists for models based on state abstraction (or state aggregation)
~\citep{bean1987aggregation,bertsekas1989adaptive,dean1997model,dietterich2000hierarchical,jong2005state,li2006towards,jiang2015abstraction}.
The main idea of state abstraction is to group together similar states and solve the reduced MDP (exactly or approximately).
Solving the optimization problem in the reduced MDP requires far fewer iterations or samples, which improves convergence speed and data efficiency.
In contrast to state abstraction, in the Bottleneck Simulator MDP the grouping is applied only within the approximate transition model while the agent's policy operates on the observed state.
Compared to state aggregation, this approach reduces the impact of compounding errors due to inaccurate abstractions in the approximate transition model.
It also allows a deep neural network policy to learn its own high-level, distributed representations of the state from scratch.
Finally, the Bottleneck Simulator MDP structure allows us to perform a mathematical analysis of the trade-offs incurred by the learned transition model, which is not possible in the general case of an arbitrary transition model.

In a related vein, learning a factorized MDP (for example, by factorizing the state transition model) has also been investigated extensively in the literature~\citep{boutilier1999decision,degris2006learning,strehl2007efficient,ross2008model,bellemare2013bayesian,wu2014model,NIPS2014_5445,hallak2015off}.
For example, \citet{ross2008model} develop an efficient Bayesian framework for learning factorized MDPs.
As another example, \citet{bellemare2013bayesian} propose a Bayesian framework for learning a factored environment model (transition model) based on a class of recursively decomposable factorizations. % of the transition model 

%propose an efficient algorithm for learning

\textbf{Dialogue Systems}:
Much work has applied reinforcement learning to training or improving dialogue systems.
The idea that dialogue can be formulated as a sequential decision making problem based on a Markov decision process (MDP) appeared already in the 1990s for goal-oriented dialogue systems~\citep{singh1999reinforcement,singh2002optimizing,williams2007partially,young2013pomdp,paek2006reinforcement,henderson2008hybrid,pieraccini2009we,svgk15}.

One line of research in this area has focused on learning dialogue systems through simulations using abstract dialogue states and actions~\citep{eckert1997user,levin2000stochastic,chung2004developing,cuayahuitl2005human,georgila2006user,schatzmann2007agenda,heeman2009representing,traum2008multi,georgila2011reinforcement,lee2012pomdp,khouzaimi2017incremental,lopez2016automatic,su2016continuously,fatemi2016policy,asri2016sequence}.
The approaches here differ based on how the simulator itself is created or estimated, and whether or not the simulator is also considered an agent, which is trying to optimize its own reward.
For example, \citet{levin2000stochastic} tackle the problem of building a flight booking dialogue system.
They estimate a user simulator model by counting transition probabilities between dialogue states and user actions (similar to an n-gram model), which is then used to train a reinforcement learning policy.
In their setting, the states and actions are all abstract discrete variables, which minimizes the amount of natural language understanding and generation the policy has to learn.
As another example, \citet{georgila2011reinforcement} tackle the problem of learning dialogue policies for negotiation games, where each party in the dialogue is an agent with its own reward function.
In their setting, each policy is in effect also a user simulator, and is trained by playing against other policies using model-free on-policy reinforcement learning.
As a more recent example, \citet{yu2016strategy} build a open-domain, chitchat dialogue system using reinforcement learning.
In particular, \citet{yu2016strategy} propose to learn a dialogue manager policy through model-free off-policy reinforcement learning based on simulations with the template-based system A.L.I.C.E.~\citep{wallace2009anatomy} with a reward function learned from crowdsourced annotations. This is shown to yield substantial improvements w.r.t.\@ both the overall appropriateness of each system response and the conversational depth of the dialogues (e.g.\@ how long the system remains on topic).

Researchers have also recently started to investigate learning generative neural network policies operating directing on raw text through user simulations~\citep{li2016deep,das2017learning,lewis2017dealornodeal,liu2017iterative,lewis2017dealornodeal}.
In contrast to earlier work, these policies require both a deeper understanding of natural language and an ability to generate natural language.
For example, \citet{li2016deep} propose to train a generative sequence-to-sequence neural network using maximum log-likelihood, and then fine-tune it with a multi-objective function. The multi-objective function includes, among other things, a reinforcement learning signal based on self-play Monte Carlo rollouts (i.e.\@ simulated trajectories are generated by sampling from the model, similar to~\citep{silver2016mastering}) using a hand-crafted reward function.
\citet{lewis2017dealornodeal} apply model-free reinforcement learning for learning a system capable of negotiation in a toy domain from crowdsourced data. They demonstrate that it's feasible to learn an effective policy by training a generative sequence-to-sequence neural network on crowdsourced data, and that the policy can be further improved using on-policy reinforcement learning through self-play and Monte Carlo rollouts.
Both \citet{li2016deep} and \citet{lewis2017dealornodeal} use self-play.
Self-play is a viable option for training their policies because their problems are symmetric in the policy space (e.g.\@ any policy performing well on one side of the negotiation game will also perform well on the other side).
In contrast, self-play is unlikely to be an effective training method in our case, because the interactions are highly asymmetric: human users speak differently to our system than they would to humans and, further, they expect different answers.
\citet{liu2017iterative} use model-free on-policy reinforcement learning to improve a system in a restaurant booking toy domain. For training the system policy, they employ a user simulator trained on real-world human-human dialogues. In particular, under the constraint that both the system and the user share the exact same reward function, they demonstrate that reinforcement learning can be used to improve both the system policy and the user simulator. 
In a related vein, \citet{zhao2016towards} learn an end-to-end neural network system for playing a quiz game using off-policy reinforcement learning, where the environment is a game simulator. They demonstrate that combining reinforcement learning with dialogue state tracking labels yields superior performance.

In all previous work on dialogue systems, user simulators have been defined as rule-based models (e.g.\@ A.L.I.C.E.\@), stochastic models on the states and actions (e.g.\@ n-gram models, generative neural networks), or a combination of the two.
To the best of our knowledge, this is the first work to consider learning a transition model based on abstractions. %through abstractions of the transition model. % in the state space transition. % work is the first to learn a transition model over abstract states.
%In most cases, given a user simulator, the collected training data is discarded and the policy is learned directly from simulations with the user simulator.
%In contrast, the Bottleneck Simulator MDP that we propose is a non-parametric approach, which repeatedly uses the collected training data during policy training.

